Fidelity-Weighted Learning

Training deep neural networks requires many training samples, but in practice training labels are expensive to obtain and may be of varying quality, as some may be from trusted expert labelers while others might be from heuristics or other sources of weak supervision such as crowd-sourcing. This creates a fundamental quality versus-quantity trade-off in the learning process. Do we learn from the small amount of high-quality data or the potentially large amount of weakly-labeled data? We argue that if the learner could somehow know and take the label-quality into account when learning the data representation, we could get the best of both worlds. To this end, we propose "fidelity-weighted learning" (FWL), a semi-supervised student-teacher approach for training deep neural networks using weakly-labeled data. FWL modulates the parameter updates to a student network (trained on the task we care about) on a per-sample basis according to the posterior confidence of its label-quality estimated by a teacher (who has access to the high-quality labels). Both student and teacher are learned from the data. We evaluate FWL on two tasks in information retrieval and natural language processing where we outperform state-of-the-art alternative semi-supervised methods, indicating that our approach makes better use of strong and weak labels, and leads to better task-dependent data representations.

==> Images/table_sentiment_res.tex <==
\begin{table}[tbp]

% Can remove this if space is not an issue.
\scriptsize

\centering
\caption{\label{tbl_main_sent}\fontsize{8}{7}\selectfont{Performance of the proposed \fwl approach and baseline methods for sentiment classification task. 
\ps{i} indicates that the improvements with respect to the baseline\#$i$ are statistically significant, at the 0.05 level using the paired two-tailed t-test, with Bonferroni correction.}}
\vspace{-5pt}
\begin{adjustbox}{max width=0.47\columnwidth}
\begin{tabular}{r l l l}
\toprule
& Method & SemEval-14 & SemEval-15
\\ \midrule
1 & \small{WA$_\text{Lexicon}$} 
& 0.5141 & 0.4471
\\ \midrule
2 & \small{NN$_{\text{W}}$} 
& 0.6719\ps{13} & 0.5606\ps{1} 
\\
3 & \small{NN$_{\text{S}}$} 
& 0.6307\ps{1} & 0.5811\ps{12}
\\ \midrule
4 & \small{NN$_{\text{S}^+\text{/W}}$} 
& 0.7032\ps{123} & 0.6319\ps{123}
\\
5 & \small{NN$_{\text{W} \to \text{S}}$} 
& 0.7080\ps{123} & 0.6441\ps{123}
\\
6 & \small{NN$_{\text{W}^\omega \to \text{S}}$} 
& 0.7166\ps{1234} & 0.6603\ps{12345}
\\ \midrule
7 & \small{NN$_{\text{W} \to \mathcal{GP}_{\text{w/o}~c}}$} 
& 0.7202 \ps{12345} & 0.6590\ps{12345}
\\
8 & \small{\fwl} 
& \textbf{0.7470} \ps{1234567} & \textbf{0.6830}\ps{1234567}
\\ \midrule
9 & \small{SemEval$^\text{Best}$} 
& 0.7162 & 0.6618
\\
& & \tiny{\citep{Rouvier:2016}} & \tiny{\citep{Deriu2016:SemEval}}
\\\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-10pt}
\end{table}

==> trash.tex <==


% \section{Introduction1}
% \label{sec:introduction}

% The success of deep neural networks to date
% %in computer vision~\citep{krizhevsky2012imagenet}, natural language processing~\citep{collobert2008unified}, and information retrieval~\citep{welling2005exponential}
% depends strongly on the availability of labeled data which is costly and not always easy to obtain. 
% Usually it is much easier to obtain small quantities of high-quality labeled data and large quantities of unlabeled data. The problem of how to best integrate these two sources of information  during training is an active pursuit in the field of semi-supervised learning~\citep{chapelle2009semi}. However, for a large class of tasks it is also easy to define one or more ``\was'', additional (albeit noisy) sources of \emph{weak supervision} based on heuristics or ``weaker'', biased classifiers trained on e.g.\ non-expert crowd-sourced data or data from different (but related) domains. This additional data is easy and cheap to generate, but it is not immediately clear if and how these additional weakly labeled data can be used to train a stronger classifier.

% In practice, machine learning systems may also be provided with data samples of variable quality. For example, in a large dataset of images only a small fraction of samples may be labeled by experts and the rest may be crowd-sourced using e.g.\ Amazon Mechanical Turk~\cite{Veit:2017}. In addition, in some applications, labels are intentionally perturbed due to privacy issues~\citep{wainwright2012privacy}. When this weak supervision is inexpensive to obtain, the simplest approach is to simply expand the training set by including the weakly supervised instances.  For instance, it has recently been shown that a small amount of expert-labeled data can be augmented by a large set of raw data with labels coming from a heuristic function~\citep{Dehghani:2017:SIGIR}. 

% In this work, inspired by Vapnik's \emph{learning using privileged information} (LUPI)~\citep{vapnik2009new, vapnik2015learning}, we propose a method to effectively make use of information from a small set of correctly labeled data to improve the performance of a semi-supervised learning algorithm.  The main idea behind LUPI comes from the fact that humans learn much faster than machines. One reason it advocates for this discrepancy is the role that an \emph{Intelligent Teacher} plays in human learning. In this framework the training data is a collection of triplets
% \begin{equation}
%     \{(x_1, x_1^*, y_1),\ldots,(x_n,x_n^*,y_n)\}\mathtt{\sim}P^n(x,x^*,y)
% \end{equation}
% where each ${(x_i,y_i)}$ is a pair of feature-label and $x_i^*$ is the additional information provided by an intelligent teacher to ease the learning process. Additional information for each ${(x_i,y_i)}$ is available only during training time and the learning machine must only rely on $x_i$ at test time. The theory of LUPI studies how to leverage such a teaching signal $x_i^*$ to outperform learning algorithms utilizing only the normal features $x_i$. For example, MRI brain images can be augmented with high-level medical or even psychological descriptions of Alzheimer's to build a classifier that predicts the probability of Alzheimer's disease from an MRI image at test time.

% %It is known from statistical learning theory~\citep{vapnik1998statistical} that the following bound for test error is satisfied with probability $1-\delta$
% %\begin{equation}
% %\label{eq:LUPI_error_bound}
% %    R(f) \leq R_n(f) + O\left(\left(\frac{|H|_{VC}-\log %\sigma}{n}\right)^\alpha\right),
% %\end{equation}
% %where $R_n(f)$ denotes the training error over $n$ instances and $\alpha \in [0.5,1]$. When the classes are not $separable$, $\alpha = 0.5$ meaning that the machine learns at a slow rate of $O(n^{-1/2})$. For easier problems where classes are $separable$, $\alpha=1$ resulting in a learning rate of $O(n^{-1})$.  The difference between these two cases is severe. The same error bound achieved for a separable problem with 10 thousands data points is only obtainable for a non-separable problem when 100 million data points are provided. This is prohibitive even when large datasets are not so costly. 

% In this paper, we propose a \emph{teacher}-\emph{student} framework for semi-supervised learning. In our setup, we build on the LUPI formulation where a student is supposed to solve the main prediction task while the intelligent teacher provides additional information to improve its learning. In addition, our formulation includes a third module named the \emph{intern}, which is used by both student and teacher. The intern is supposed to learn the appropriate representation for the task and its output is used as inputs to the other two modules.
% We validate our intuitions on a toy task, and then consider two real-world tasks: relevance ranking from information retrieval and sentence sentiment classification from natural language processing. For both tasks, we have a large set of unlabeled samples along with a heuristic function which is able to assign a weak label to each sample. Inevitable inaccuracies in designing the heuristic function causes noisy labels. Finally, we are also given samples which are labeled by field experts whose labels are trusted. \mosi{instead of this, I would say: ``which are labeled by field experts whose labels can be considered as the observations from the underlying true function.''
% because we have this assumption that there could be some small noise (but unstructured, like cases of annotators disagreement!) in these labels and the GP kernel is selected based on this assumption (and this assumption improves the results!)}

% We then design the components of our leaning system as follows: The \emph{student} is implemented as a neural network. It is doing the main job in our framework, which is solving the task at test time. The \emph{teacher}, implemented as a Gaussian process, knows the quality of the labels and gives this additional (privileged) information to the student during training. Finally, the \emph{intern} is the main workhorse of our system which is employed by both teacher and student during training and by the student at test time. The implementation is detailed in section~\ref{sec:implementation}. 

% The theory of LUPI was first developed and proved for support vector machines by Vapnik as a means for knowledge transfer. Hinton introduced~\emph{Dark knowledge} as a spiritually close idea in the context of neural networks~\citep{Hinton:2006}. He proposed to use a large network or an ensemble of networks for training and a smaller network at test time. It turned out that compressing knowledge of a large system into a smaller system can improve the generalization ability of the smaller system. It was shown in~\citep{lopez2015unifying} that dark knowledge and LUPI can be unified under a single umbrella, called \emph{generalized distillation}. The core idea of these models is \emph{machines-teaching-machines}. As the name suggests, a machine (in our case, student neural network) is learning the knowledge embedded in another machine (the teacher network). Our framework extends this idea in the following directions:

% \begin{itemize}
%     \item Trainable teacher: It is often assumed that the teacher in LUPI framework has some additional true information. We show that when this extra information is not available, one can still use the LUPI setup and define an implicit teacher whose knowledge is learned from the true data.
%   \item Bayesian teacher: The proposed teacher is Bayesian. It provides posterior uncertainty of the labels of each instance.
%   \item Intern: We introduce an intern module which learns a mutual embedding (representation) for both student and teacher. This is in particular interesting because it defines a two-way channel between the teacher and the student.
%   \item Scalable teacher: We propose a scalable method for the teacher to acquire its knowledge by a method called clustered Gaussian process.
% \end{itemize}





% \section{Connection with optimization with noisy gradients}

% [REMOVE?]

% Another perspective to our work is from optimization perspective. To keep the introduction brief, we postpone this exposition to the Appendix.
% %
% Weak supervision can be studied in optimization level where it results in noisy gradients. \citet{schaul2013no} proposed a method to set the learning rate adaptively by estimating first and second order statistics of gradients which requires hessian information. 
% \citet{song2015learning} proposed a method to determine the learning rate and order of samples to minimize the final regret.  This method requires numerical optimization to determine the learning rate which is prohibitive especially when the number of noise levels is numerous. 
% %
% Due to the nature of our setup, the noise level is continuous but the cause of noise is known. Therefore we propose a method to take advantage of this known noise model to avoid computing the statistics of gradients. 
% Our method is defined as an outer loop over normal optimization procedure and does not need estimating the hessian information or numerical optimization required for setting the learning rate for each iteration.

% When a set of data points with true and noisy labels is at hand, semi-supervised learning methods such as fine-tuning may help. This is usually done by pre-training a model by weak samples then fine tuning it by observations from the true function samples~\citep{Dehghani:2017:SIGIR, Severyn:2015:SIGIR}.
% The downside is that such approaches treat labels as a binary set \{True, Noisy\} and are oblivious to the amount of noise in the labels. 
% Simply speaking, they do not consider the cause of noise in the labels and only focus on the effect. 
% However, in our model, we try to estimate the pattern of the noise in the label which leads to a more stable fine tuning.
% %
% More similar to our proposed method are noise-aware models where the distribution of noise in the labels is estimated while training is being carried out~\citep{Patrini:2016, Sukhbaatar:2014}. Our work extends this line of work to situations where the cause of noise is explicitly available.

% We propose a Bayesian semi-supervised method that leverages a small amount of data with true labels along with a large amount of data with weak labels. We take on a causal approach by directly looking into the cause of label noise when it is available. This information is embedded in several stages of our model.
% %
% In the class of problems that we consider, the cause of label noise is the inaccuracy in a heuristic labeling function. We propose a setting consisting of two main modules called \tnet which is in charge of learning a suitable representation and performing the main task, and \nest which shapes the learning process.  
% %
% In the first stage, \tnet is pre-trained by a large set of weakly annotated instances to learn the representation of the data and the main task (Figure ~\ref{fig:step1}). The learned representation maps each instance into a point in the suitable feature space for the main task.
% %
% Then, while enjoying the data representation learned in the previous step, \nest is trained on a small set of observations with true labels.
% This order of training enables \nest to absorb information of the cause and polish up that information by the observations with true labels
% %It is noteworthy that \nest implicitly absorbs information of weak labels as it is fed by the the representation of data learned, down stream of the main task, based on the weak labels
% (Figure(~\ref{fig:step2})).
% %
% In the last stage, for each data instance (either in unlabeled or labeled set), we generate a pair of $\langle label, confidence\rangle$ using \nest. This new set of weakly labeled points augmented with corresponding confidence scores is used to fine tune \tnet (Figure(~\ref{fig:step3})).


